Chameleon: Adaptive Code Optimization for Expedited Deep Neural Network Compilation

Achieving faster execution with shorter compilation time can foster further diversity and innovation in neural networks. However, the current paradigm of executing neural networks either relies on hand-optimized libraries, traditional compilation heuristics, or very recently genetic algorithms and other stochastic methods. These methods suffer from frequent costly hardware measurements rendering them not only too time consuming but also suboptimal. As such, we devise a solution that can learn to quickly adapt to a previously unseen design space for code optimization, both accelerating the search and improving the output performance. This solution dubbed Chameleon leverages reinforcement learning whose solution takes fewer steps to converge, and develops an adaptive sampling algorithm that not only focuses on the costly samples (real hardware measurements) on representative points but also uses a domain-knowledge inspired logic to improve the samples itself. Experimentation with real hardware shows that Chameleon provides 4.45x speed up in optimization time over AutoTVM, while also improving inference time of the modern deep networks by 5.6%.

==> body/challenges.tex <==
\section{Challenges and Design Objectives}
\label{sec:motivation}
\vspace{-0.1in}

\subsection{Challenges}
\vspace{-0.05in}
%
Even with the advances from prior works~\cite{TVM,TC,AutoTVM}, optimizing compilation can be around 10 hours for ResNet-18 with 12 convolution layers.
%
This long optimization time gets more prominent in deeper or wider networks with models with more larger layers to optimize.
%
Such long optimization time results from naive stochastic search of simulated annealing or genetic algorithm and excessive number of real hardware measurements from simple sampling.
%
Therefore, having large and diverse enough design space provided a priori, variables that determine the effectiveness of the optimizing compiler can be narrowed down to two subproblems: (1) developing an efficient search algorithm, and (2) reducing the number of times the compiler reaches for real hardware measurements.

\vspace{-0.05in}
\subsection{Design Objectives}
\label{sec:design_goals}
\vspace{-0.05in}
%
\paragraph{Improving efficacy of search algorithm.}
%
One strategy to approach this problem is to do a brute force search.
%
However, when the design space could be as large as $10^{10}$, optimization becomes too time-consuming or it fails to provide a reasonable solution.
%
Another strategy is to incorporate random search~\cite{TVM} or genetic algorithms~\cite{TC,TVM,COGA,COGA2} to enhance efficiency of the search.
%
Prior works~\cite{AutoTVM, SAComp, DRESC} have also used simulated annealing in the context of compiler optimization problem because it statistically guarantees finding an optimal solution.

Although previous work~\cite{TVM} finds reasonable configurations with the interplay of simulated annealing and cost models with boosted trees, simulated annealing is known for its slow speed and could be an overkill.
%
Furthermore, simulated annealing is oblivious to the gradual changes in the cost model and naively trusts the estimation, leaving room for improvement in the effectiveness of the search.
%
This calls for a more intelligent search algorithm ($\mathcal{A}^*$) that meets following objectives:
%
%\vspace{-0.2in}
\begin{align}
	s_\Theta^* = \argmax_{s_\Theta \subset \mathcal{S}_\Theta} \big( P(f_{ideal}(\tau) - \max_{\Theta \in s_\Theta}f(\tau(\Theta)) = 0 \big) \label{eq:search_explore} \\
	\mathcal{A}^* = \argmin_{\mathcal{A}} \big( \#steps(s_{\Theta,t} \leftarrow \mathcal{A}(s_{\Theta,t-1})) = s_{\Theta*} \big) \label{eq:search_exploit}
\end{align}
%
Equation~\ref{eq:search_explore} finds a set of samples ($s_{\Theta}$) that maximizes the probability of achieving ideal performance ($f_{ideal}$) for a given code ($\tau$) on the hardware ({\em exploration}), and Equation~\ref{eq:search_exploit} encourages finding an algorithm that minimizes search steps by maximizing the reuse of information from previous set of samples ($s_{\Theta,t-1}$) ({\em exploitation}). 
%
In this work, we explore a new possibility using reinforcement learning that strikes a good balance between {\em exploration} and {\em exploitation} during the search.
%
In the rest of the paper, we call this the search agent, and we address this in Section \ref{sec:exploration_agent}.

\vspace{-0.05in}
\paragraph{Reducing number of costly hardware measurements.}
%
Figure~\ref{fig:compile_time} presents the total and the breakdown of the time it takes to optimize convolution layers of ResNet-18.
%
It is clear from the graph that majority of the compile time is spent on reaching for measurements on real hardware that is used as a feedback for the aforementioned search algorithms.
%
Therefore, reducing the frequency of hardware measurements will reduce the overall optimization time significantly.
%
In prior work~\cite{AutoTVM}, search algorithms pick fixed number of samples per iteration and takes a greedy approach in determining which configurations to measure on the real hardware.
%
However, such method overlook the distribution of the samples while making such decision, which not only leads to longer optimization time from excessive number of hardware measurements but also leaves room for more effective exploration.

Therefore, the goal of this work is to methodically vary the number of configuration samples to measure with regard to the distribution of the samples ($s_{\Theta} = \{\Theta_1, \Theta_2, ..., \Theta_3\}$) and to intelligently deduce representative points ($s_{\Theta}' \subset \mathcal{S}_\Theta$) within the design space of configurations that would subsume the subspace ($s_{\Theta} \subset \mathcal{S}_\Theta$).
%
Therefore, there are two conflicting goals of methodically and intelligently sampling from the distribution to minimize measurements, yet maximize both the potential information ($\mathcal{H}_\Theta$) and the overall fitness ($f$) of configuration samples.
%
Given, ($\mathcal{S}_\Theta, s_\Theta, f, \tau$), our problem can be formalized into following two conflicting objectives:
%
\begin{align}
	s_\Theta' = \argmin_{s_\Theta \subset \mathcal{S}_\Theta} |s_\Theta| \qquad \text{vs.} \qquad s_\Theta' = \argmax_{s_\Theta \subset \mathcal{S}_\Theta} \big( \sum_{\Theta \in s_\Theta} (\mathcal{H}_\Theta) \cdot \min_{\Theta \in s_\Theta}f(\tau(\Theta)) \big)
	\label{eq:sample}
\end{align}
%
Figure~\ref{fig:clustering} plots the distribution of sampled configurations by reducing to two dimensions, the observation is that subsets of the sampled configurations are clustered.
%
Since, the variance of their performance is relatively small despite performance differences among configurations), it is inefficient for the compiler to make measurements on all configurations from each cluster.
%
We leverage this observation and methodically sample representative configurations from the distribution of configurations from the search agent to make our compiler make less hardware measurements without compromising the quality of compilation.
%
We address this issue in Section~\ref{sec:sampling_module}.

\begin{figure}[t]
  \vspace{-0.1in}
  \begin{minipage}{.48\textwidth}
    \vspace{-0.31in}
    \includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{figs/compile_time.pdf}
    \vspace{-0.2in}
    \caption{AutoTVM optimization time for ResNet-18 on \titan. Numbers in bars denote fraction of time for measurements.}
    \label{fig:compile_time}
  \end{minipage}
  \hfill
  \begin{minipage}{.48\textwidth}
    \vspace{-0.065in}
    \subfigure[VGG-16 4th layer]{\includegraphics[width=0.495\linewidth]{figs/clustering/cluster_2_new.pdf}}
    \subfigure[ResNet-18 11th layer]{\includegraphics[width=0.495\linewidth]{figs/clustering/cluster_1_new.pdf}}
    \vspace{-0.15in}
    \caption{Illustration of clusters visible among distribution of samples during optimization.\newline\newline}
    \label{fig:clustering}
  \end{minipage}
  \vspace{-0.25in}
\end{figure}
